Optomechanical cavities based on epitaxial GaP on nominally (001)-oriented Si

Gallium phosphide (GaP) has recently received considerable attention as a suitable material for building photonic integrated circuits due to its remarkable optical and piezoelectric properties. Usually, GaP is grown epitaxially on III-V substrates to keep its crystallinity and later transferred to silicon wafers for further processing. Here, an alternative promising route for the fabrication of optomechanical (OM) cavities on GaP epitaxially grown on nominally (001)-oriented Si is introduced by using a two-step process consisting of a low-temperature etching of GaP followed by selective etching of the underneath silicon. The low-temperature (-30 $^o$C) during the dry-etching of GaP hinders the lateral etching rate, preserving the pattern with a deviation between the design and the pattern in the GaP layer lower than 5 %, avoiding the complex process of transferring and bonding a GaP wafer to a silicon-on-insulator wafer. To demonstrate the quality and feasibility of the proposed fabrication route, suspended OM cavities are fabricated and experimentally characterized. The cavities show optical quality factors between 10$^3$ and 10$^4$, and localized mechanical resonances at frequencies around 3.1 GHz. Both optical and mechanical resonances are close to those previously reported on crystalline GaP structures. These results suggest a simple and low-cost way to build GaP-based photonic devices directly integrated on industry-standard Si(001) photonic wafers.

==> erased.tex <==

% Please provide Biographies and photos for Essays, Feature Articles, Progress Reports, Reviews, and Perspectives for those authors who should be highlighted  
% These should be at most 100 words long
% For other article types this section can be removed
% Photographs should be 40mm broad and 50 mm high

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}



% Table of contents entry should be 50 - 60 words long
% Image should be 55 mm broad and 50 mm high or 110 mm broad and 20 mm high


\begin{figure}
\textbf{Table of Contents}\\
\medskip
  \includegraphics{toc-image.png}
  \medskip
  \caption*{ToC Entry}
\end{figure}

